Constrained Auto-Regressive Decoding Constrains Generative Retrieval

Generative retrieval seeks to replace traditional search index data structures with a single large-scale neural network, offering the potential for improved efficiency and seamless integration with generative large language models. As an end-to-end paradigm, generative retrieval adopts a learned differentiable search index to conduct retrieval by directly generating document identifiers through corpus-specific constrained decoding. The generalization capabilities of generative retrieval on out-of-distribution corpora have gathered significant attention. In this paper, we examine the inherent limitations of constrained auto-regressive generation from two essential perspectives: constraints and beam search. We begin with the Bayes-optimal setting where the generative retrieval model exactly captures the underlying relevance distribution of all possible documents. Then we apply the model to specific corpora by simply adding corpus-specific constraints. Our main findings are two-fold: (i) For the effect of constraints, we derive a lower bound of the error, in terms of the KL divergence between the ground-truth and the model-predicted step-wise marginal distributions. (ii) For the beam search algorithm used during generation, we reveal that the usage of marginal distributions may not be an ideal approach. This paper aims to improve our theoretical understanding of the generalization capabilities of the auto-regressive decoding retrieval paradigm, laying a foundation for its limitations and inspiring future advancements toward more robust and generalizable generative retrieval.

==> Figures/constraints_10k_non_uniform.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/Resource/constraints_10k.non_uniform_sampling.exponential_score.T2.pdf}
    \caption{The KL divergence error in the first generation step.
    A subset of top-$10,000$ rank list from SLIM++~\citep{liSLIM2023} is treated as the complete corpus, and the downstream corpus is sampled with the \emph{same} relevance distribution.}
    \label{fig:constraints_10k_non_uniform}
\end{figure}


==> Figures/constraints_10k_uniform.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/Resource/constraints_10k.uniform_sampling.pdf}
    \caption{The KL divergence error in the first generation step on downstream corpus.
    A subset of top-$10,000$ rank list from SLIM++~\citep{liSLIM2023} is treated as the complete corpus, and the downstream corpus is uniformly sampled.}
    \label{fig:constraints_10k_uniform}
\end{figure}



==> Figures/constraints_full_non_uniform.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/Resource/constraints_full.non_uniform_sampling.pdf}
    \caption{The KL divergence error in the first generation step on MS MARCO V1 passage corpus.
    The relevance distribution is constructed as Section~\ref{sub:setup}.
    The downstream corpus sampled with the \emph{same} relevance distribution.}
    \label{fig:constraints_full_non_uniform}
\end{figure}



==> Figures/constraints_full_uniform.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/Resource/constraints_full.uniform_sampling.pdf}
    \caption{The KL divergence error in the first generation step on MS MARCO V1 passage corpus.
    The relevance distribution is constructed as Section~\ref{sub:setup}.
    The downstream corpus uniformly sampled.}
    \label{fig:constraints_full_uniform}
\end{figure}



==> Tables/vocab-size-relation.tex <==
\begin{table}[ht]
\caption{The relation of vocabulary size $k$ and \ac{bpt} and \ac{docid} length $m$.}
\label{table:vocab-size}
\begin{tabular}{ll}
    \toprule
    \textbf{Symbol} & \multicolumn{1}{c}{\textbf{Description}}
    \\
    \midrule
    $k,\,m$         & the vocabulary size and document length \\

    \bottomrule
\end{tabular}
\end{table}
